Scanning HTML at Tens of Gigabytes per Second on ARM Processors

Modern processors have instructions to process 16 bytes or more at once. These instructions are called SIMD, for single instruction, multiple data. Recent advances have leveraged SIMD instructions to accelerate parsing of common Internet formats such as JSON and base64. During HTML parsing, they quickly identify specific characters with a strategy called vectorized classification. We review their techniques and compare them with a faster alternative. We measure a 20-fold performance improvement in HTML scanning compared to traditional methods on recent ARM processors. Our findings highlight the potential of SIMD-based algorithms for optimizing Web browser performance.

==> code/chromium/stuff.tex <==


\begin{verbatim}
 // character.
 template <typename T, typename VectorT>
   requires(sizeof(T) == 1)
 HWY_ATTR ALWAYS_INLINE ClassifiedValue
 SimdAdvanceAndClassify(const T*& start,
                        const T* end,
                        VectorT low_nibble_mask,
                        VectorT high_nibble_mask) {
   namespace hw = hwy::HWY_NAMESPACE;
   DCHECK_GE(static_cast<size_t>(end - start), kVectorizationThreshold);

   hw::FixedTag<uint8_t, 16> tag;
   static constexpr auto stride = hw::MaxLanes(tag);

   const auto low_nib_and_mask = hw::Set(tag, 0xf);

   // The main scanning loop.
   for (; start + (stride - 1) < end; start += stride) {
     const auto input = hw::LoadU(tag, reinterpret_cast<const uint8_t*>(start));
     if (const auto result = TryMatch(tag, input, low_nibble_mask,
                                      high_nibble_mask, low_nib_and_mask);
         result.Matched()) {
       start = reinterpret_cast<const T*>(start + result.index_in_vector);
       return result.classified_value;
     };
   }

   // Scan the last stride.
   if (start < end) {
     const auto input =
         hw::LoadU(tag, reinterpret_cast<const uint8_t*>(end - stride));
     if (const auto result = TryMatch(tag, input, low_nibble_mask,
                                      high_nibble_mask, low_nib_and_mask);
         result.Matched()) {
       start = end - stride + result.index_in_vector;
       return result.classified_value;
     }
     start = end;
   }

   return 0;
 }
\end{verbatim}

\begin{verbatim}
template <typename D, typename VectorT>
 HWY_ATTR ALWAYS_INLINE MatchedCharacter TryMatch(D tag,
                                                  VectorT input,
                                                  VectorT low_nibble_mask,
                                                  VectorT high_nibble_mask,
                                                  VectorT low_nib_and_mask) {
   namespace hw = hwy::HWY_NAMESPACE;

   const auto nib_lo = input & low_nib_and_mask;
   const auto nib_hi = hw::ShiftRight<4>(input);

   const auto shuf_lo = hw::TableLookupBytes(low_nibble_mask, nib_lo);
   const auto shuf_hi = hw::TableLookupBytes(high_nibble_mask, nib_hi);

   const auto classified = shuf_lo & shuf_hi;

   if (const intptr_t index =
           hw::FindFirstTrue(tag, classified != hw::Zero(tag));
       index != -1) {
     return {static_cast<size_t>(index), hw::ExtractLane(classified, index)};
   }
\end{verbatim}

\begin{verbatim}
template <class D>
intptr_t FindFirstTrue(D d, MFromD<D> mask) {
  const uint64_t nib = detail::NibblesFromMask(d, mask);
  if (nib == 0) return -1;
  constexpr size_t kDiv = 4 * sizeof(TFromD<D>);
  return static_cast<intptr_t>(Num0BitsBelowLS1Bit_Nonzero64(nib) / kDiv);
}
\end{verbatim}

\begin{verbatim}
// Returns mask[i]? 0xF : 0 in each nibble. This is more efficient than
// BitsFromMask for use in (partial) CountTrue, FindFirstTrue and AllFalse.
template <class D, HWY_IF_V_SIZE_D(D, 16)>
HWY_INLINE uint64_t NibblesFromMask(D d, MFromD<D> mask) {
  const Full128<uint16_t> du16;
  const Vec128<uint16_t> vu16 = BitCast(du16, VecFromMask(d, mask));
  const Vec64<uint8_t> nib(vshrn_n_u16(vu16.raw, 4));
  return GetLane(BitCast(Full64<uint64_t>(), nib));
}
\end{verbatim}

